TE2Rules: Explaining Tree Ensembles using Rules

Tree Ensemble (TE) models, such as Gradient Boosted Trees, often achieve optimal performance on tabular datasets, yet their lack of transparency poses challenges for comprehending their decision logic. This paper introduces TE2Rules (Tree Ensemble to Rules), a novel approach for explaining binary classification tree ensemble models through a list of rules, particularly focusing on explaining the minority class. Many state-of-the-art explainers struggle with minority class explanations, making TE2Rules valuable in such cases. The rules generated by TE2Rules closely approximate the original model, ensuring high fidelity, providing an accurate and interpretable means to understand decision-making. Experimental results demonstrate that TE2Rules scales effectively to tree ensembles with hundreds of trees, achieving higher fidelity within runtimes comparable to baselines. TE2Rules allows for a trade-off between runtime and fidelity, enhancing its practical applicability. The implementation is available here: https://github.com/linkedin/TE2Rules.

==> checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations of our method in Section \ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not foresee any negative societal impact from our work on explaining AI models.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We do not have any theoretical results}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{We do not have any theoretical results}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will add the code and the instructions needed to reproduce the main experimental results in supplemental material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our method is deterministic}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We have discussed compute resources in Section \ref{sec:results}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{All the datasets used in our work are open source}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All the datasets used in our work are open source}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not use any human subjects/crowdsourcing}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We did not use any human subjects/crowdsourcing}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We did not use any human subjects/crowdsourcing}
\end{enumerate}


\end{enumerate}





==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ |c|c|c| } 
% 			\hline
% 			Notation & Description  \\ \hline \hline
% 			TE & Tree Ensemble  \\ 
% 			T & Number of Trees in TE  \\ 
% 			D & Maximum Depth of a Tree in TE  \\ 
% 			F & Number of attributes  \\ 
% 			$f_{t}(x)$ & Score for instance $x$ from $t^{th}$ tree in TE  \\
% 			$f_{TE}(x)$ & Prediction for instance $x$ from TE  \\ 
% 			\hline
% 			IDS & Interpretable Decision Set  \\ 
% 			L & Number of Decision clauses in an IDS \\
% 			$f_{IDS}(x)$ & Prediction for instance $x$ from IDS  \\
% 			$r$ & A Decision clause in IDS  \\ 
% 			$s$ & Score of an intermediate Decision clause  \\ 
% 			CR & Constituent Decision clauses  \\ 
% 			CT & Constituent Trees  \\ 
% 			\hline
% 		\end{tabular}
% 		\caption{Notations}
% 		\label{table:notations}
% 	\end{center}
% \end{table}

We are given a binary TE classifier with $T$ trees. The TE makes classifications according to
  \begin{equation}
    f_{TE}(x) = 
    \begin{cases}
      1, & \text{if } \sum_{t=1}^{T} w_t f_t(x) + b > c \\
      0, & \text{otherwise}
    \end{cases}
  \end{equation}
where $w_t$ is the weight of tree $t$, $b$ is a bias term, and $c$ is the decision threshold of the TE. We decompose the TE with a RL by searching for high-precision rules for one of the labels (e.g. $f_{TE}(x) = 1$), until most instances with the label is covered by at least one rule from the RL. All the uncovered instances are assigned the other label. 

The RL should satisfy the following three properties: it should mimic the TE for most inputs (\emph{high fidelity}): $f_{TE}(x) \approx f_{RL}(x)$, where
  \begin{equation}
    f_{RL}(x) = 
    \begin{cases}
      1, & \text{if x satisfies at least 1 rule from the RL} \\
      0, & \text{otherwise.}
    \end{cases}
  \end{equation}
Moreover, the RL should be short and its rules should be simple enough to be comprehensible by humans (\emph{high interpretability}). Finally, the algorithm should converge in a short run-time even when explaining large datasets and high-complexity TE models (\emph{high scalability}).

The RL is evaluated for two tasks: (i) global-level model decomposition: explain or substitute the TE with a high-fidelity and interpretable RL, and (ii) instance-level outcome explanation: explain each individual instance with a high-precision, high-recall and interpretable rule.

% The ensemble can be trained either using bagging (Random Forest) or boosting (Gradient Boosted Trees, Adaptive Boosting). The tree consists of internal nodes which make splits on some feature being greater or less than some split value. Each leaf node of the tree contains a value. The tree scores a data sample $x$ as the value of the leaf node that $x$ belongs to. The score of TE is a linear combination of the scores from each tree using some weights $w_t$ and a bias $b$. The final prediction made by the TE $f_{TE}(x)$ is based on a threshold on the TE score. Without loss of generality, we can assume that the threshold is $0$. $f_{TE}(x) = sign(\sum_{t=1}^{T} w_t f_t(x) + b)$
	
% Our formulation of TE is general enough to describe tree ensembles trained using both bagging and boosting framework. Boosting frameworks often train a weighted linear combination of trees directly. In bagging frameworks, often the leaf nodes of the trees assign a class directly without assigning a value and the final decision is taken based on a majority voting by all the trees in the ensemble. Such ensembles can be reformulated in our approach by assigning leaf nodes with binary values of $0$ or $1$ based on the binary class decision made by the leaf and setting bias $b = -T/2$. Hence, for some data sample $x$, if and only if more than $T/2$ out of $T$ trees in the ensemble vote for class $1$, $f_{TE}(x) = 1$.

% Interpretable Decision Set (IDS) is a set of decision subspaces where each decision subspace $r_i$ is defined by an intersection of feature subspaces, i.e. $r_i = (x_{j_1}\in a)\cap(x_{j_2}\in b)\cap(x_{j_3}\in c)$. 
% \begin{center}
% 	$\mathbf{IDS = \cup_{i-1}^{L} r_i}$ 
% \end{center}

% IDS can be used as a binary classifier as follows: 
% \begin{center}
% 	$\mathbf{f_{IDS}(x) = 1 \iff x \in IDS}$. 
% \end{center}

% Our goal is to generate an IDS that has the same prediction as $f_{TE}(x)$ for all $x$. 


